Minibatch Selection for Language Models via Partition Matroid Constrained Gradient Matching

Training large language models (LLMs) on heterogeneous data requires selecting minibatches that balance convergence speed with coverage across domains. Existing methods either select samples independently within each domain or rely on computationally expensive proxy models to learn continuous domain weights. We propose PartitionSel, a cross-domain minibatch selection approach that maximizes a validation-guided gradient-matching utility under per-domain budgets encoded as a partition-matroid constraint. By coupling the per-domain budgets through a single utility, PartitionSel is designed to reduce redundancy in selections across domains. The proposed objective is weakly submodular and admits an orthogonal matching pursuit algorithm with provable approximation guarantees. Empirically, we evaluate PartitionSel for minibatch selection during the fine-tuning of Qwen2.5 and Llama-3 on MetaMathQA and Mol-Instructions. PartitionSel achieves robust gains over per-domain and domain-agnostic baselines on both benchmarks. It also reduces the number of conflicting gradient pairs within each batch, indicating that the cross-domain coupling translates into more compatible training updates.

==> icml2026/motivation_fig.tex <==

\begin{figure}[t!]
    \centering
    \begin{minipage}{0.49\columnwidth}
        \centering
        \includegraphics[scale=0.33]{icml2026/figures/mini_batch_domains.png}
        \vspace{-0.6em}
        {\scriptsize Independent per-domain selection}
    \end{minipage}%
    \begin{minipage}{0.49\columnwidth}
        \centering
        \includegraphics[scale=0.33]{icml2026/figures/mini_batch_domains_less_overlap.png}
        \vspace{-0.6em}
        {\scriptsize Joint selection ($\methodprop$)}
    \end{minipage}%
    
\includegraphics[width=0.85\columnwidth]{icml2026/figures/mini_batch_legend.png}
    \vspace{-0.8em}
    \caption{\textbf{Distribution across domains per batch.} 
    \textit{Samples near the intersection of two domains exhibit high gradient similarity.} 
    Each bar shows the final selected samples (icons denote individual samples). 
    (\emph{Left}: Independent per-domain selection leads to redundant selections, over-representing boundary samples across domains. 
    \emph{Right}: Our method, $\methodprop$, jointly selects samples across domains, thereby reducing redundancy.)
    }
    \label{fig:motivation}
\end{figure}
